End-to-End Table Question Answering via Retrieval-Augmented Generation

Most existing end-to-end Table Question Answering (Table QA) models consist of a two-stage framework with a retriever to select relevant table candidates from a corpus and a reader to locate the correct answers from table candidates. Even though the accuracy of the reader models is significantly improved with the recent transformer-based approaches, the overall performance of such frameworks still suffers from the poor accuracy of using traditional information retrieval techniques as retrievers. To alleviate this problem, we introduce T-RAG, an end-to-end Table QA model, where a non-parametric dense vector index is fine-tuned jointly with BART, a parametric sequence-to-sequence model to generate answer tokens. Given any natural language question, T-RAG utilizes a unified pipeline to automatically search through a table corpus to directly locate the correct answer from the table cells. We apply T-RAG to recent open-domain Table QA benchmarks and demonstrate that the fine-tuned T-RAG model is able to achieve state-of-the-art performance in both the end-to-end Table QA and the table retrieval tasks.

==> 5analysis.tex <==
\section{The Application of \projName}
To further validate \projName\ and solve \task\ problems in real-world scenarios, we built an end-to-end \task\ system based on \projName. The user interface of the system is shown in Figure~\ref{fig.screenshot}. The system allows users to pre-load any table corpus they are interested in for querying them. Once the tables are loaded, \projName\ takes two inputs from users: (1) any natural language questions; (2) an optional $k$ value to determine the size of the retrieved answers. If $k$ is not given, it is set as 4 by default. In the example presented in Figure~\ref{fig.screenshot}, we input the question ``Who played the first Phantom of the Opera?'' from NQ-TABLES and set $k$ as 4. As output, \projName\ retrieves the top answers and 
the corresponding tables. The top-ranked tables are displayed with a heatmap highlighting the answer cells. 
\begin{figure}
\centering 
\includegraphics[width=0.9\linewidth]{fig/aaai_screenshot.pdf}
\caption{A screenshot of the user interface of \projName.} 
\label{fig.screenshot}
\vspace{-3 mm}
\end{figure}
